Single-Qubit Gates Beyond the Rotating-Wave Approximation for Strongly Anharmonic Low-Frequency Qubits

Single-qubit gates are in many quantum platforms applied using a linear drive resonant with the qubit transition frequency which is often theoretically described within the rotating-wave approximation (RWA). However, for fast gates on low-frequency qubits, the RWA may not hold and we need to consider the contribution from counter-rotating terms to the qubit dynamics. The inclusion of counter-rotating terms into the theoretical description gives rise to two challenges. Firstly, it becomes challenging to analytically calculate the time evolution as the Hamiltonian is no longer self-commuting. Moreover, the time evolution now depends on the carrier phase such that, in general, every operation in a sequence of gates is different. In this work, we derive and verify a correction to the drive pulses that minimizes the effect of these counter-rotating terms in a two-level system. We then derive a second correction term that arises from non-computational levels for a strongly anharmonic system. We experimentally implement these correction terms on a fluxonium superconducting qubit, which is an example of a strongly anharmonic, low-frequency qubit for which the RWA may not hold, and demonstrate how fast, high-fidelity single-qubit gates can be achieved without the need for additional hardware complexities.

==> circuits/circuit1.tex <==
\begin{quantikz}[column sep=10pt, row sep={17pt,between origins}]
    \lstick{$| 0 \rangle$} & \qw & \gate{X_\pi}\gategroup[1,steps=2,style={inner
sep=6pt}]{$M$ repetitions} & \gate{X_\pi} & \qw & \meter{x}
\end{quantikz}

==> circuits/circuit3.tex <==
\begin{quantikz}[column sep=10pt, row sep={17pt,between origins}]
    \lstick{$| 0 \rangle$} & \qw & \gate{X_\pi}\gategroup[1,steps=4,style={inner
sep=6pt}]{$M$ repetitions} & \gate{Z} & \gate{X_\pi} & \gate{Z} & \qw & \meter{y}
\end{quantikz}
